Dr.ICL: Demonstration-Retrieved In-context Learning

In-context learning (ICL), teaching a large language model (LLM) to perform a task with few-shot demonstrations rather than adjusting the model parameters, has emerged as a strong paradigm for using LLMs. While early studies primarily used a fixed or random set of demonstrations for all test queries, recent research suggests that retrieving semantically similar demonstrations to the input from a pool of available demonstrations results in better performance. This work expands the applicability of retrieval-based ICL approaches by demonstrating that even simple word-overlap similarity measures such as BM25 outperform randomly selected demonstrations. Furthermore, we extend the success of retrieval-based ICL to instruction-finetuned LLMs as well as Chain-of-Thought (CoT) prompting. For instruction-finetuned LLMs, we find that although a model has already seen the training data at training time, retrieving demonstrations from the training data at test time yields better results compared to using no demonstrations or random demonstrations. Last but not least, we train a task-specific demonstration retriever that outperforms off-the-shelf retrievers.

==> experiments_old.tex <==
\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/plots_flanpalm_one.png}
\caption{One-shot inference with three types of demonstrations, random, BM25, and GTR. 
}
% For the few shots of BM25 and GTR, we use 8 shots for GSM8k and 5 shots for the rest of the tasks. 
% In both one-shot and few-shot cases, retrieved demonstrations are more effective than random demonstrations.}
\label{fig:palm_offshelf}
\end{figure*}

\begin{figure*}[t]
\centering
\includegraphics[width=\linewidth]{figures/plots_flanpalm_few.png}
\caption{Few-shot inference with three types of demonstrations, random, BM25, and GTR. 
% For the few shots of BM25 and GTR, we use 8 shots for GSM8k and 5 shots for the rest of the tasks. 
In both one-shot and few-shot cases, retrieved demonstrations are more effective than random demonstrations.}
\label{fig:palm_offshelf_fewshot}
\end{figure*}

\section{Experiments}

\paragraph{Datasets and Evaluation Metrics}
We study varies tasks across 5 datasets: free-form question answering (NQ), natural language inference (ANLI-r3), mathematical reasoning (GSM8k and AQuA) and boolean question answering (StrategyQA).
For the last three datasets, we apply CoT. 
All the tasks are evaluated by exact matching accuracy. % We include four tasks: question answering (NQ), natural language inference (ANLI r1/2/3), context-sensitive meaning representations (WiC), and mathematical reasoning (GSM8k) with CoT. All the tasks are evaluated by exact matching accuracy.

\paragraph{Large Language Models}

PaLM-540B~\cite{chowdhery2022palm} and Flan-PaLM(540B)~\cite{chung2022scaling} are used as the primary LLMs. Both models have the same architecture, but Flan-PaLM has been further trained on thousands of tasks for instruction learning and shows superior generalization performance compared to PaLM.
% Results from experiments on Flan-PaLM indicate the ongoing value of the training data, as it can be used not only to train a model, but also at inference time as a retrieval corpus to find the most representative demonstrations to construct in-context.
In the inference time, we use the temperature of 0.0 and max decoding length 10 for most tasks except for GSM8k, which uses decoding length of 256 as the model also generates the CoT.

\paragraph{Retrievers} 
We examine two off-the-shelf retrievers: BM25~\cite{robertson2009probabilistic} and GTR~\cite{ni2021large}. 
GTR is a dual-encoder type retriever (based on T5) that is trained on the MS Marco dataset~\cite{nguyen2016ms}; we use the base-GTR for all the experiments. 
We then train a demonstration retriever initiated from GTR on the collected data described in \S\ref{sec:training}, named as Demo-GTR. We firstly use pretrained GTR to retrieve 100 demonstrations candidates, and then use PaLM-62B to get the score of each candidate for the sake of efficient scoring process. 
Then we select the top-5 reranked demonstrations as the positive candidates to train GTR. 
We find that using the hard-negative does not yield difference compared to only using the in-batch negative.

\paragraph{Retrieval Strategy}
We create separate retrieval corpora for each task using the associated training data. 
For the tasks with CoT, each entry in the corpus is composed of the question, the CoT, and the answer, while for other tasks are without the CoT. 
During inference, given a testing query, the most similar entries are retrieved as the demonstrations. 

\subsection{Results}

\paragraph{Off-the-shelf-retriever performance}
Figure \ref{fig:palm_offshelf} and Figure \ref{fig:palm_offshelf_fewshot} show the performance of PaLM and Flan-PaLM under one-shot and few-shot ICL settings, with and without retrievers. 
We have the following observations. 
% Firstly, while previous research has demonstrated the effectiveness of retrieval-demonstrations in few-shot scenarios, we observe that it also enhances the one-shot ICL performance. Moreover, the improvement in the one-shot scenario is more significant than the few-shot scenario. Specifically, for GTR, the average improvement is 4.38 in the one-shot scenario compared to 3.5 in the few-shot scenario. Similarly, for BM25, the average improvement is 4.08 in the one-shot scenario, but the improvement in the few-shot scenario is X.
% Secondly, we find that for factoid question answering and classification tasks, GTR outperforms BM25. However, for mathematical tasks requiring reasoning, BM25 is more effective than GTR. 
% % Interestingly, we observe that BM25 retrieves longer (more reasoning steps) demonstrations than GTR.   
% This observation might indicate that more complex demonstrations is more helpful for learning mathematical reasoning tasks. \citet{fu2022complexity} shows that the demonstrations with more reasoning steps are more helpful in mathematical reasoning task, our finding serves as an additional support for such a claim. 

\textit{Observation 1: BM25, a simple word-overlapping retriever, is capable of finding more effective demonstrations than random ones.} 
In contrast to previous work by ~\citep{liu2022makes}, which employed semantic sentence encoders to find demonstrations, we use BM25 to find the demonstrations and show that it improves the performance over using random demonstrations.
Compared to other retrievers like GTR or sentence encoders, BM25 is more efficient in terms of indexing memory and retrieval latency, which makes it easier to deploy \dricl{} in real-world applications. 

\textit{Observation 2: \dricl{} always improves one-shot ICL.} 
While previous research has demonstrated the effectiveness of retrieval-demonstrations in few-shot scenarios, we observe that it also enhances the one-shot ICL performance. Moreover, the improvement in the one-shot scenario is more significant than the few-shot scenario. Specifically, for GTR, the average improvement is 4.38 in the one-shot scenario compared to 3.5 in the few-shot scenario. Similarly, for BM25, the average improvement is 4.08 in the one-shot scenario, but the improvement in the few-shot scenario is X.

\textit{Observation 3: \dricl{} not always improves few-shot ICL.} 
\textcolor{red}{Here, we will add some diversity analysis.}

\textit{Observation 4: \dricl{} can further improve advanced prompting technique, Chain-of-Thought.}
In our experiment with the mathematical reasoning task, GSM8k, we investigate if \dricl{} can improve CoT prompting further. We observe that using \dricl{} in conjunction with CoT result in improved performance leveraging both BM25 and GTR under one-shot and few-shot ICL scenarios. This finding suggests that \dricl{} has the potential to enhance the performance of powerful prompting techniques.  

% \textit{Observation 4: While GTR retrieves more representative demonstrations than BM25 for factoid question answering and classification tasks, BM25 is more effective for complex mathematical task with CoT.} 
% Based on our results of five datasets for question answering and classification tasks, we find that GTR outperforms BM25 in retrieving more representative demonstrations. However, for complex mathematical tasks involving CoT, BM25 shows to be more effective. We notice that BM25 retrieves longer demonstrations with more reasoning steps than GTR, which could suggest that more complex demonstrations are beneficial for learning mathematical reasoning tasks.

\input{tables/flan}
\textit{Observation 5: \dricl{} also improves instruction-finetuned LLM.}
% Lastly, our results with an instruction-finetuned LLM, i.e. Flan-PaLM~\citep{chung2022scaling}, indicates that training data can be useful not only for training a model but for accompanying a retriever for testing, suggesting a maximum way to utilizing training data which are expensive to collect.
Previous research has primarily focused on investigating retrieval-demonstrations ICL with general LLMs (such as GPT-3) rather than instruction-finetuned LLMs, possibly because they did not consider reusing the training data. In our study, we examine ReD-ICL using an instruction-finetuned LLM, Flan-PaLM, and present the performance results in Table \ref{tab:flan_withoutft}. Overall, the retrieved demonstrations outperform no demonstrations or random demonstrations. This implies that the training data should be reused during inference as they can be retrieved and enhance the performance, even if the model has already seen such data. We conjecture that the retrieved demonstrations may enhance knowledge localization for ICL, which could explain the observed improvement.


% \medskip
% \input{tables/flan}
% \noindent Previous research has primarily focused on investigating retrieval-demonstrations ICL with general LLMs (such as GPT-3) rather than instruction-finetuned LLMs, possibly because they did not consider reusing the training data. In our study, we examine ReD-ICL using an instruction-finetuned LLM, Flan-PaLM, and present the performance results in Table \ref{tab:flan_withoutft}. Overall, the retrieved demonstrations outperform no demonstrations or random demonstrations. This implies that the training data should be reused during inference as they can be retrieved and enhance the performance, even if the model has already seen such data. We conjecture that the retrieved demonstrations may enhance knowledge localization for ICL, which could explain the observed improvement.

\medskip
\noindent In summary, the aforementioned results hold significant value for real-world applications, as incorporating a retriever into the inference pipeline can greatly enhance the ICL performance of LLM. This is particularly true with BM25, which is highly effective at a large scale for both inference latency and indexing memory.
% Even with simple BM25 retriever, the performance of retrieved-demonstrations are better than random demonstrations.
% Since BM25 is both inference and indexing efficient at large scale, it makes retrieved-demonstrations ICL with LLM an appealing real-world applications. 

\paragraph{Trained Demonstration Retriever Performance} 
\input{tables/palm_train_retriever}
We experiment our trained demonstration retriever with PaLM.
Table \ref{tab:palm_trained_retriever} displays both one-shot and few-shot performance and show that the demonstration retriever is better than the-off-shelf GTR in a majority of the cases and achieves better overall performance. 
Notably, the improvements were most significant in the one-shot ICL scenario, which requires less inference latency and computing resources than few-shot ICL. These promising results suggest that the trained retriever could provide an effective alternative to off-the-shelf models. 
% This suggests that our proposed method is effective to find the better top 1 demonstration, but it is insufficient the find the better combination of few shots. We leave this as a future work. 

==> meeting_notes.tex <==
\subsection{Last Meeting Notes} 

Who are the audience of the paper 
\begin{itemize}
    \item Users of Large language models with training data for a specific task: for example utilize GPT-3 for business purposes.
        \begin{itemize}
            \item Finetune, rely on OpenAI finetuning API.
            \begin{itemize}
                \item  People are worried about data privacy and security. Is our approach safer? Our approach is not necessarily safer. OpenAI still see your in-context examples.
                \item Our approach is easier to use because it doesn't rely on the finetune/PEFT API. Is FT API more expensive? Yes: After FT, they (OpenAI) have to server your model. Very expensive.
            \end{itemize}
            \item Prompt engineering.
                \begin{itemize}
                    \item What is wrong with prompt engineering? Too complicated.
                    \item Can our method work with prompt engineering? $1+1>1$?
                    \begin{itemize}
                        \item We need experiments and try on all "those" PE variantions.
                    \end{itemize}
                \end{itemize}
            \item **Few-shot in-context (is the simplest thing everyone should do)
                \begin{itemize}
                    \item The few-shot examples are chosen manually, with some simple heuristics (e.g., diverse enough examples).
                    \item [Current] Off-the-shelf fewshot $>$ random fewshot.
                    \item [Need] learned retriever $>$ the OTS.
                    \item [Need ablation] performance vs number of shots.
                \end{itemize}
            \item Is our approach a general solution?
                \begin{itemize}
                    \item It is better to be true. Otherwise, it is not that useful. TODO(scale number of eval tasks)
                \end{itemize}
        \end{itemize}
        \item Is our approach a general solution?
            \begin{itemize}
                It is better to be true. Otherwise, it is not that useful. TODO(scale number of eval tasks)
            \end{itemize}
    % \item Large language model designers.
    %     \begin{itemize}
    %         \item Not the main story. Just mention in the future work.
    %     \end{itemize}
\end{itemize}
What will make the paper interesting 
\begin{itemize}
    \item C4 for generation tasks and creative tasks.  
    \item Compare to prompting engineering (especially CoT): 
Retrieval can be combined with CoT or any other good prompting engineering.
\end{itemize}







==> seq_introduction.tex <==
\section{Introduction}
% Don't stop using your training data. 
% Most of the existing few-shot in-context learning use a few random demonstrations from an available training set and fix the prompt for all the testing questions. We call such strategy as fixed few-shot in-context learning. 
% An obvious shortcoming of such method is that most of the training examples are wasted. 
% On the other hand, instruction tuning utilizes the entire training data to update the model parameters. Nevertheless, in most of the existing work, such fine-tuned models do not use the training data afterwards.  
% In this work, we study dynamic few-shot in-context learning which maximizes the usage of training data. 
% [describe the method here.]

% To support this story, we need to show two sets of experiments. 
% \begin{itemize}
%     \item PaLM performance: compare with random baselines.
%     \item Flan Performance: compare with zeros-hot and random baselines. 
% \end{itemize}
% [One thing to notice is that for instruction fine-tuned LLMs, people might care more about the generalization on unseen tasks. Either we should do experiments on retrieving examples from training set for unseen testing set and show it is better than zero-shot, or we should tell the story not lead to such kind of question, and we can mention out-of-domain retrieval as a future work in the discussion section.]

Language models are now the foundation models for almost all natural language processing tasks across a wide range of domains~\citep{bommasani2021opportunities}. One important development trend in these models is scaling, where the parameters of language models increase from millions to billions~\citep{kaplan2020scaling}. The scaling law also brings emergent abilities~\citep{weiemergent} to large language models (LLMs), one of the most exciting being instruction and in-context learning (ICL)~\citep{brown2020language}. With ICL, instructions and a few demonstration examples, are provided to LLMs as in-context, allowing them to perform well on new tasks, including complex reasoning tasks like mathematical reasoning, without the need for fine-tuning.

ICL offers several advantages over the traditional training approach of language models, which involves pre-training followed by fine-tuning. One key benefit is that fine-tuning may not always be possible. For example, models may not be publicly available for fine-tuning, or may require users to share their training data, which may not be feasible due to privacy concerns. Additionally, using a fine-tuned model may require additional costs for launching with a third party. Another advantage of ICL is that it does not have the overfitting issue commonly present with fine-tuning. Since ICL does not update the model's parameters, the underlying model remains general and not specific to a particular task or data set.

While ICL is an effective approach, many existing ICL methods use fixed examples in the context for every question. Research has shown that this method is not the optimal solution and that using examples similar to the input query can lead to better performance than using random examples. We refer to this type of inference approach as Dynamic-ICL to distinguish it from the traditional fixed-ICL paradigm. Dynamic-ICL is more flexible and leads to improved results. Different questions within a task may pertain to different topics or require different reasoning skills. For example, an addition equation example would be more relevant to solving an addition equation than a subtraction equation example.

In this work, we first demonstrate that Dynamic-ICL indeed consistently improve Fixed-ICL by experimenting two retrieval methods on a X tasks with Y LLMs. 
More importantly, we propose a method to sequentially retrieve demonstrations.   
Our intuition is that a good set of in-context demonstrations should provide comprehensive and well-rounded understanding of the subject, and thus 
when we retrieve a demonstration, it should complement or add to the already existing representative demonstrations to enhance the overall understanding of the topic or problem being discussed.
However, existing retrievers do not have this capability. Thus, we train a new retriever to retrieve similar but diverse examples. We begin by creating a training set. To identify examples that are similar to the input question but also distinct from prior examples, we use the signal of a language model. Given an input question, the correct answer, and a few examples, we prepend these examples to the input question and retrieve the top-k new examples. We then concatenate these new examples with the prior examples and prepend them to the input question. We provide this sequence to the language model and score the ground truth of the input question. Finally, we sort the top-k examples by their corresponding scores and use the top-N and bottom-N examples as positive and hard-negative examples, respectively. The training objective of the retriever is to maximize the score of the positive example among the hard-negative and in-batch negative examples, given the prior examples and the question.

Our experiments demonstrate that this retrieval method is effective in obtaining a balance of similar and diverse examples. Using these examples, we show that the performance of PaLM and Flan-PaLM is significantly improved compared to using random or only-similar examples.



==> sequential_retrieval.tex <==
\subsection{Sequential Demonstration Retriever}
We consider few-shot scenario, where a set of demonstrations are provided as in-context. 
% Ideally, a good demonstration in the context bring extra explicit information to $LM$ such that the probability of $y_{q}$ increase. 
Previous Retrievers retrieve demonstrations based on $x_{q}$, and thus the top-n demonstrations are likely similar to each others.
We aim to build a retriever such that the retrieved demonstrations are representative but also bring extra positive effects on $LM$ compared to only using the prior demonstrations.
With this goal, we propose a sequential retrieval process, such that each $d_i$ is retrieved based on $x_q$ and the previous demonstrations $C_{i-1} = \{d_1, \cdots, d_{i+1}\}$. 
\begin{equation}
    d_{i} = Retriever(x_q, C_{i-1}, 1)
\end{equation}
To quantity the effect of $d$ on $LM$ given a set of previous demonstrations $C$, we use the perplexity as bellows,  
\begin{align}
    P(y_q) &= LM(C, x_q)\\
    P(y_q)^{'} &= LM(C+d, x_q) \\
    \Delta &= P(y_q)^{'} - P(y_q)
\end{align}
$d$ adds a positive effect on $C$ compared to $C$ if $\Delta$ is larger than 0. 

\paragraph{Obtain the training data}
Empirically, due to the large cost of employ a LLM (e.g. 540B) to get the score of ground truth, we leverage a relatively small LM (e.g. 64B). 
\paragraph{Training}
We employ GTR as the initial retriever. And then train GTR on our prepared training data using in-batch negative and contrastive learning objective. 
\begin{equation}
    \mathcal{L}_{con} = -\log \frac{e^{\mathrm{sim}(v_{q}, v_{d^{+}})}}{e^{\mathrm{sim}(v_{q}, v_{d^{+}})}+ \sum_{j=1}^{j=n}e^{\mathrm{sim}(v_{q}, v_{d_{j}^{-}}})},
    \label{eq:dpr_loss1}
\end{equation}
where $v_{q}$ is the representation of input text and $v_{d}$ for the demonstration, and $\mathrm{sim}(q, c)$ is the inner-dot product.
The negative demonstrations include the positive demonstrations for the other input text in the same batch and 1 hard negative demonstrations. 



==> tables/flan.tex <==
% \begin{table}[t]
%     \centering
%     \small
%     \resizebox{0.95\linewidth}{!}{
%     \setlength{\tabcolsep}{5pt}
%     \begin{tabular}{@{}cccc@{}}
%         \toprule
%         \textbf{Task}  & \textbf{Method} & \textbf{One Shot} & \textbf{Few Shots} \\
%         \toprule
%     \multirow{3}{*}{{NQ }} 
   
%     & Random    & 45.3  & 45.8 \\
%     % & BM25      & -  \\
%     & GTR       & 47.3  & 48.3\\
%     \midrule
%     \multirow{3}{*}{{ANLI (r3)}}
%      & Random    & 60.83  & 64.58\\
%     % & BM25      & - \\
%     & GTR       & 62.58  & 65.17\\
%     \midrule
%     \multirow{3}{*}{{GSM8k}}
%      & Random    & 68.2 & 70.7 \\
%     % & BM25      & 70.5 \\
%     & GTR       & 71.2 & 70.2 \\
   
%     \bottomrule
%     \end{tabular}
%     }
%     \caption{Performance of Flan-PaLM with three types of demonstrations on three datasets in one-shot and few-shots scenario. 5 demonstrations are used for NQ and ANLI3 in the few-shot case, and 8 demonstrations for GSM8k. Retrieved demonstrations are more effective than random demonstrations, showing the ongoing value of training data in the testing time. 
%     }
%     \label{tab:flan_withoutft} 
% \end{table}
        
\begin{table}[t]
    \centering
    \small
    \resizebox{0.95\linewidth}{!}{
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{@{}cccc@{}}
        \toprule
        \textbf{Task}  & \textbf{Method} & \textbf{One Shot} & \textbf{Few Shots} \\
        \toprule
    \multirow{3}{*}{{NQ }} 
   
    & Random    & 45.3  & 45.8 \\
    & BM25      & 45.9  & 47.0 \\
    & GTR       & \textbf{47.3}  & \textbf{48.3}\\
    \midrule
    \multirow{3}{*}{{ANLI (r3)}}
     & Random    & 64.0  & 70.1 \\
    & BM25      & 68.0 & 69.5 \\
    & GTR       & \textbf{68.8}  & \textbf{70.6} \\
    \midrule
    \multirow{3}{*}{{GSM8k}}
     & Random    & 68.2 & {70.7} \\
    & BM25      & 70.5 & \textbf{72.0} \\
    & GTR       & \textbf{71.2} & 70.2 \\
    \midrule
   \multirow{3}{*}{{StrategyQA}}
     & Random    & 82.1 & 81.2 \\
    & BM25      & \textbf{82.6} & \textbf{82.6} \\
    & GTR       & 81.2 & 82.1 \\
    \midrule
    \multirow{3}{*}{{AQUA}}
     & Random    & 43.3 & 44.9 \\
    & BM25      & \textbf{54.3} & \textbf{54.7} \\
    & GTR       & 53.1 & 54.3 \\
    \midrule
    \multirow{3}{*}{{ECQA}}
     & Random    & \textbf{84.0} & \textbf{87.1} \\
    & BM25      & 81.7 & 84.4 \\
    & GTR       & 83.6 & 84.4 \\
    \bottomrule
    \end{tabular}
    }
    \caption{Flan-PaLM: Xin's number. 
    }
    \label{tab:flan_withoutft2} 
\end{table}


\begin{table}[t]
    \centering
    \small
    \resizebox{0.95\linewidth}{!}{
    \setlength{\tabcolsep}{5pt}
    \begin{tabular}{@{}cccc@{}}
        \toprule
        \textbf{Task}  & \textbf{Method} & \textbf{One Shot} & \textbf{Few Shots} \\
        \toprule
    \multirow{3}{*}{{GSM8K}}
    & Random    &  57.5 & 60.0 \\
    & BM25      & \textbf{58.3} &\textbf{ 61.2} \\
    & GTR       & 54.4 & - \\
    \midrule
   \multirow{3}{*}{{StrategyQA}}
     & Random    &  71.0 & 72.0 \\
    & BM25      & \textbf{73.4} & \textbf{76.8} \\
    & GTR       & 71.5 & 75.8 \\
    \midrule
    \multirow{3}{*}{{AQUA}}
     & Random    & 26.0 & 32.7 \\
    & BM25      & 44.9 & 42.9 \\
    & GTR       & \textbf{46.5} & \textbf{43.3} \\
    \midrule
    \multirow{3}{*}{{ECQA}}
     & Random    & \textbf{69.7} & \textbf{75.4} \\
    & BM25      & 67.6 & 73.1 \\
    & GTR       & 68.7 & 72.8 \\
    \bottomrule
    \end{tabular}
    }
    \caption{PaLM: Xin's number. 
    }
    \label{tab:palm_withoutft2} 
\end{table}
        

==> tables/old_examples.tex <==
\begin{table*}[t]
    \centering 
    \small
    \setlength{\tabcolsep}{3pt}
    % \resizebox{\linewidth}{!}{
    \begin{tabular}{@{}p{0.32\linewidth}p{0.32\linewidth}p{0.32\linewidth}@{}}
        \toprule 
        \textbf{Question} & \textbf{BM25 Demo} & \textbf{GTR Demo} \\
        \toprule
        Q: when does the new episodes of supernatural start? \newline A: October 12, 2017
        & 
        Q: when does the new episodes of ghost adventures start? \newline A: June 16, 2018
        & 
        Q: when does the next episode of supernatural come out? \newline A: April 5, 2018\\
        \midrule
        Q: Train ‘A’ leaves Mumbai Central for Lucknow at 11 am, running at the speed of 40 kmph. Train ‘B’ leaves Mumbai Central for Lucknow by the same route at 2 pm on the same day, running at the speed of 72 kmph. At what time will the two trains meet each other?
        \newline Options:
        (A) 12 am on the next day
        (B) 5 am on the next day
        (C) 5 pm on the next day
        (D) 2 pm on the next day
        (E) None of these
        \newline Step-by-step reasoning process: Distance covered by train A before the train B leaves
        Mumbai Central = 40 x 3 = 120 km
        Time taken to cross each other = 120/12 = 10 hours
        Required time = 2pm + 10 = 12 am on the next day
        \newline
        A: (A)
        & 
        Q: A train leaves Mumabai at 9 am at a speed of 40 kmph. After one hour, another train leaves Mumbai in the same direction as that of the first train at a speed of 60 kmph. When and at what distance from Mumbai do the two trains meet?
        \newline Options:
        (A) 187
        (B) 279
        (C) 120
        (D) 278
        (E) 379
        \newline Step-by-step reasoning process: When the second train leaves Mumbai the first train covers 40 * 1 = 40 km
        So, the distance between first train and second train is 40 km at 10.00am
        Time taken by the trains to meet
        = Distance / relative speed = 40 / (60 -40) = 2 hours
        So, the two trains meet at 12 a.m. The two trains meet 2 * 60 = 120 km away from Mumbai.
        \newline
        A: (C)
        & 
        Q: A train leaves Mumabai at 9 am at a speed of 40 kmph. After one hour, another train leaves Mumbai in the same direction as that of the first train at a speed of 50 kmph. When and at what distance from Mumbai do the two trains meet?
        \newline Options:
        (A) 2:00pm, 206 km
        (B) 2:00pm, 220 km
        (C) 2:00pm, 200 km
        (D) 2:00pm, 208 km
        (E) 2:00pm, 230 km
        \newline Step-by-step reasoning process: When the second train leaves Mumbai the first train covers 40 * 1 = 40 km
        So, the distance between first train and second train is 40 km at 10.00am
        Time taken by the trains to meet
        = Distance / relative speed
        = 40 / (50 -40) = 4 hours
        So, the two trains meet at 2 p.m. The two trains meet 4 * 50
        = 200 km away from Mumbai.
        \newline
        A: (C)\\
        \midrule
        % Q: What does a person in ISIS practice?
        % \newline Options:
        % - boredom
        % - terrorism
        % - meanness
        % - stupidity
        % - ridiculous
        % \newline Step-by-step reasoning process: ISIS is a jihadist group with particularly violent ideologies
        % People working in the ISIS are often terrorists
        % Terrorists tend to practice terrorism
        % \newline 
        % A: terrorism 
        % & 
        % Q: A person who yawns and paces to help pass the time is likely feeling what?
        % \newline Options:
        % - ridiculous
        % - excitement
        % - meanness
        % - terrorism
        % - boredom
        % \newline Step-by-step reasoning process: People tend to yawn when they have sleepy and have nothig to do
        % Pacing to help pass time means the person has nothing to do
        % People who are bored, often yawn and pace to pass time
        % \newline A: boredom
        % &
        % Q: What are you hoping to do when listening to an expert speak?
        % \newline Options:
        % - learning
        % - fatigue
        % - mercy
        % - empathy
        % - anxiety
        % \newline Step-by-step reasoning process: Experts teach us various lessons
        % We consult expert when we want to learn something
        % \newline A: learning \\
        % \midrule
        Q: Could the Pope be on an episode of Pimp My Ride?
        \newline Step-by-step reasoning process:
        Pimp My Ride is a show where people's cars are upgraded and improved The Pope has a personal vehicle called the Popemobile.
        \newline A: yes
        &
        Q: Can every digit in Pi be memorized?
        \newline Step-by-step reasoning process: The digits of Pi are infinite.The human mind cannot hold an infinite amount of information.
        \newline A: no
        &
        Q: Can a false pope become a saint?
        \newline Step-by-step reasoning process: A false pope, or antipope, is someone that tries to claim they are the true pope but the church rejects them. Hippolytus (c. 170–235 AD) headed a schismatic group as a rival to the Bishop of Rome, thus becoming an antipope. Hippolytus (c. 170–235 AD) was named a saint in the Roman Catholic Church.
        \newline A: yes\\
        \bottomrule
    \end{tabular}
    % }
    \caption{
    Examples of retrieved demonstrations.
    NQ, AQUQ, StrategyQA}
    \label{tab:example}
\end{table*}


